On the duration and intensity of cumulative advantage competitions

The role of skill (fitness) and luck (randomness) as driving forces on the dynamics of resource accumulation in a myriad of systems have long puzzled scientists. Fueled by undisputed inequalities that emerge from actual competitions, there is a pressing need for better understanding the effects of skill and luck in resource accumulation. When such competitions are driven by externalities such as cumulative advantage (CA), the rich-get-richer effect, little is known with respect to fundamental properties such as their duration and intensity. In this work we provide a mathematical understanding of how CA exacerbates the role of luck in detriment of skill in simple and well-studied competition models. We show, for instance, that if two agents are competing for resources that arrive sequentially at each time unit, an early stroke of luck can place the less skilled in the lead for an extremely long period of time, a phenomenon we call "struggle of the fittest". In the absence of CA, the more skilled quickly prevails despite any early stroke of luck that the less skilled may have. We prove that duration of a simple skill and luck competition model exhibit power law tails when CA is present, regardless of skill difference, which is in sharp contrast to exponential tails when CA is absent. Our findings have important implications to competitions not only in complex social systems but also in contexts that leverage such models.

==> TEX/ack.tex <==
%%!TEX PS-program = pdflatexmk
%%!TEX root = ../main.tex

\section{Acknowledgments}
This work was supported in part by NSF grant CNS-1065133, Army Research Office Con-
tract W911NF-12-1-03, and ARL Cooperative Agreement W911NF-09-2-0053.
%The views and conclusions contained in this document are those of the authors and should not be interpreted as representing the official policies, either expressed or implied of the NSF, ARL, or the U.S. Government. The U.S. Government is authorized to reproduce and distribute reprints for Government purposes notwithstanding any copyright notation hereon.
D. Figueiredo received financial support through grants from CAPES, FAPERJ and CNPq (Brazil).
Liyuan Sun was supported in part by the National Natural Science Foundation  (61221063), 863 High Tech Development Plan (2012AA011003) and 111 International Collaboration Program, of China.

==> TEX/intro-old.tex <==
%%!TEX PS-program = pdflatexmk
%%!TEX root = ../main.tex
\section{Introduction}
\label{sec:intro}

The distribution of requests for resources has direct impact on the performance of computational and communication systems that rely or operate on such resources. Searching on P2P networks, caching in content-driven networks, advertisement placement in online social networks, and item ranking in recommendation systems, are all tasks whose performance heavily depend on how requests are distributed among various objects. Thus, leveraging and predicting how requests for resources accumulate can lead to enhanced system performance. But how do they accumulate? 

%At the same time, there is overwhelming empirical evidence that resource accumulation in a variety of social and complex systems lead to remarkable inequalities in resource distribution. 
%Examples are abundant: household wealth and income~\cite{Piketty2014}, scholarly citations~\cite{SollaPrice76,wang2013quantifying}, webpage and hashtag popularity~\cite{Barab99,Broder2000,Kwak2010}, and number of friends and followers in online social networks~\cite{Kwak2010,Ugander2011,Kumar2010}. 
%
%the contexts of mutual fund returns~\cite{FAMA:2010km}, protein binding~\cite{PRL_Eisenberg03}, 
%scholarly citations~\cite{wang2013quantifying}, sports games~\cite{Connolly:2008}, 
%scientific career longevity~\cite{Petersen2011}, and social reward systems~\cite{van2014field}. 
%
Skill (fitness) and luck (randomness) are believed to be two fundamental ingredients that drive resource request 
accumulation dynamics in a variety of social and complex systems. Apart from them, externalities are also believed 
to play a fundamental role in how requests for resources accumulate\footnote{In order to shorten the terminology requests for resources 
are treated as resources, leading to resource accumulation.}.
In this regard, cumulative advantage (CA), where accumulated resources promote gathering even 
more resources,\footnote{This phenomenon appears in the literature under many variants such as Price's
cumulative advantage model~\cite{SollaPrice76}, preferential attachment \cite{Barab99,Bianc01,Barab12}, ``the rich get richer'', Matthew effect \cite{Merton68,diprete2006cumulative,Perc2014}, and path-dependent increasing returns \cite{Arthur}.}
is a simple and widely-applied framework capturing the essence of network externalities, 
while random walk (RW) serves as the hallmark framework without externalities. 

These two parsimonious frameworks coupled with skill and luck have a long tradition in providing key 
insights into the process of resource accumulation, with CA, for instance, presented 
as a mechanism to help explain the presence of power-laws observed in empirical data~\cite{SollaPrice76,Rosen1981,Frank1995,Barab99,amaral2000classes,Pennock2002,Perc2014}.
It is also well-known that in both frameworks the most skilled is bound to accumulate 
more resources. But how long will it take? As John M. Keynes famously stated ``in the long run we 
are all dead'', and thus the assurance that the skilled will always prevail provides little practical insight.


%Recently, the pronounced U.S.\ income inequality has cast a debate over the mechanisms for resource 
%accumulation into the public arena with the role of skill and luck taking the spotlight~\cite{Piketty2014}. Will 
%skill prevail over luck? Can skill be rewarded deservedly in spite of great inequalities? The debate around 
%such questions are paramount to our times. Various mathematical models for competition dynamics confirm that the ``arc of compensation justice is long, but bends towards 
%the skilled''~\cite{RW,Mahm08}. But how much is long? As John M. Keynes famously stated ``in the long run we are all dead'', 
%and thus the assurance that the skilled will always prevail provides little practical insight. 

We approach this problem by considering classical, simple and well-studied theoretical models for competitions 
based on skill and luck that are either coupled with or free of cumulative advantage. We focus on two fundamental 
aspects of competitions: {\em duration} - the time required for the most skilled to overtake its competitor and 
forever enjoy undisputed leadership; {\em intensity} - the number of times competitors tie for the leadership. In 
this direction, we make the following main contributions (intuitively presented here):
\begin{enumerate}
\item
{\em Struggle of the fitness}: In the absence of CA, simple RW competition models driven by skill and 
luck are known to have short {\em duration} - competition duration follows a distribution with 
exponential tail~\cite{RW}. In the presence of CA, competitions are fundamentally different, 
possibly being very long - duration distribution exhibits a power-law tail 
with exponents that are proportional to skill differences and initial wealth. 
Thus, a slightly more skilled individual might have to hang on to the 
competition for an extremely long period of time before taking the ultimate lead, a phenomenon 
we call the ``struggle of the fittest''. 

\item
{\em Delusion of the weakest}: In the absence of CA, simple RW competition models driven by skill and 
luck are known to have weak intensity, exhibiting a distribution with exponential 
tail~\cite{RW}. In the presence of CA, when agents have different skills, intensity also exhibits 
an exponential, in sharp contrast with duration. Thus, long competitions are never intense. 
In particular, in a long competition the less skilled takes the lead very early on and 
is only overtaken by the more skilled very late in the competition, enjoying leadership 
for a long period of time, a phenomenon we call the ``delusion of the weakest''. 

\item
{\em Different is not shorter}: In the absence of CA, duration of RW competition models driven by skill 
and luck are always shorter when agents have different skills compared to when they have identical skills. In the 
presence of CA, this is fundamentally different, as competitions can be {\em longer} when agents have 
different skills compared to when they have identical skills. Thus, a competition where an agent 
is is slightly superior in skill can last much longer than when they have identical skills. However, if 
skill difference is large enough, then duration also becomes shorter compared to when they have identical 
skills. 
\end{enumerate}
All our contributions are observations from rigorous mathematical analysis of simple models driven by skill 
and luck in the presence of CA, as all results were known when CA is absent. We sustain theoretical results 
(which are sometimes asymptotic) with extensive simulations results indicating their validity across 
short timescales. Finally, despite 90 years since the basic CA model was first proposed~\cite{Polya23}, 
known as P\'olya's urn model, our work is, to the best of our knowledge, the first to characterize 
the duration and intensity distributions of CA competitions with skill. We believe our results have 
profound implications to our understanding of competitions, beyond its importance to the performance of 
systems that leverage resource distribution.

The rest of the paper is organized as follows. Section \ref{sec:related} briefly discusses the related work. Section \ref{sec:model} introduces the CA competition model. Section \ref{sec:results} presents the theoretical results, illustrated and supplemented by simulations. Section \ref{sec:proofs} provides the proofs for the theoretical results in Section \ref{sec:results}. Section \ref{sec:conclusion} concludes the paper.


